Maximum Persistency in Energy Minimization

We consider discrete pairwise energy minimization problem (weighted constraint satisfaction, max-sum labeling) and methods that identify a globally optimal partial assignment of variables. When finding a complete optimal assignment is intractable, determining optimal values for a part of variables is an interesting possibility. Existing methods are based on different sufficient conditions. We propose a new sufficient condition for partial optimality which is: (1) verifiable in polynomial time (2) invariant to reparametrization of the problem and permutation of labels and (3) includes many existing sufficient conditions as special cases. We pose the problem of finding the maximum optimal partial assignment identifiable by the new sufficient condition. A polynomial method is proposed which is guaranteed to assign same or larger part of variables than several existing approaches. The core of the method is a specially constructed linear program that identifies persistent assignments in an arbitrary multi-label setting.

==> tex/generic_alg.tex <==
\section{Generic Algorithm}\label{sec:generic_alg}
{\gray
\begin{lemma}$P \succeq Q$ \iff $Q\mu \neq \mu \Rightarrow P\mu \neq \mu$.
\end{lemma}
}
%\begin{theorem}%Let $P \succeq Q$ and $Q$ is improving for $f$. Then either $P$ is improving or $P \succneq Q$.
%\end{theorem}
%\begin{lemma}\label{lemma 4}If $P \succeq Q$ then $I-P-(I-P)Q = I-Q$.
%\end{lemma}
%\begin{proof}
%$I-P-(I-P)Q = I-P-Q-PQ = I-Q$.
%\qed
%\end{proof}
%
%

%\subsection{The Algorithm}
Let $\P$ be a class of projections closed under the product operation and commutative: $(\forall P,Q\in\P)$ $PQ = QP\in\P$. Also note that $PQ \succeq P,Q$. In this case $(\P, \succeq)$ is a join-semilattice.
\Theorem{T:nested} motivates the following generic algorithm for the semilattice $(\P,\succeq)$.
%the case when we restrict to a set of projections $\P$ that form a lattice \wrt the partial order $\succeq$. Let $$
%The maximum projection in the lattice is given by the projection $P = \prod_{Q \in \P} Q$.
\begin{itemize}
\item Start with the maximum projection $P \in \P$ (equals to $\prod_{Q \in \P} Q$).
\item 
Solve $v = \min_\mu \<(I-P\T)f,\mu\>$; Let $\O$ be the optimal facet and $\mu\in \O$.%and $\mu$ an interior point of $\O$.
%\item %If $v=0$ terminate; Else $v<0$.
\item If $P(\O) \subseteq \O$, then $\< (I-P\T)f, \mu \>  = \< (I-P\T)f, P\mu \> = \< f, (I-P) P \mu \> = 0$. Then by definition~\eqref{L-improving} $P$ is $\Lambda$-improving and we terminate. Otherwise $P(\O) \nsubseteq \O$ and by \Theorem{T:nested} $P$ is not improving and we continue.
%\item Let $Q$ be improving and $P \succeq Q$.
%\item Since $P$ is not improving it must be $P \succneq Q$.
%\item Consider $\mu' = Q\mu$. %It must be $\mu' \neq \mu$ ($\mu'$ is not in the optimal facet).
%Assume for contradiction that $\mu'$ is not in the optimal facet. 
%We then have $\<(I-P\T)f,\mu\> < \<(I-P\T)f,Q \mu\>$. It follows that $\<(I-Q\T)f,\mu\> = \<(I-P\T)f,\mu\>- \<(I-P\T)f,Q\mu\> <0$. Hence $Q$ is not improving (contradiction). Therefore any improving $Q$ must map the optimal facet $\O$ into itself.
\item Exclude all mappings that do not map $\O$ to $\O$. More precisely let $P' := \prod_{Q \preceq P \mid Q(\O) \subset \O} Q$. We have $P \succ P'$ ($\Null(P') \subsetneq \Null(P)$), at the same time it is guaranteed that for any mapping $Q$ that is improving we still have $P' \succeq Q$.
%\item If there is nothing to exclude, let $\mu' = P\mu$. Show $P(\O) \subset \O$. Then we have $\< (I-P\T)f, P\mu \> = \< f, (I-P) P \mu \> = 0$. It follows that $v=0$.
\end{itemize}
%
%
%
%
%
%We propose \Algorithm{Alg:generic} to solve the problem~\eqref{best L-improving}.
\par
\par
For the family of mappings $\P = \{P_\xi \mid \xi \in\{0,1\}^V \}$ introduced above the algorithm specializes as \Algorithm{Alg:generic}.


\begin{algorithm}
$\xi_{si} = 1$ for all $s\in\V$, $i\in\L_s$\tcc*{start with the maximum projection} % $v:=-1$; $x:=0$; $y':=y$; $\X:=\V$\;
\Repeat{}{%$v = 0$
	%Construct binary energy $\hat g$ from $f$ and $y',\, z$ by~\eqref{Pyz-bar-g-pre}\;
	%\begin{equation}\label{verification_step}
	Construct $(I-P\T_\xi) f$ according to~\eqref{richer-I-P T}\;
	Calculate%\\[-0.5em]
	\label{facet_step}
	\begin{equation}\label{facet_problem}
	v = \min_{\mu\in\Lambda} \<(I - P_\xi\T) f,\mu\>% a df sd fdsg dfsg dfsg dfgh df% & &\hspace{5cm}%
	\end{equation}
	\lIf(\tcc*[f]{found improving mapping}){v=0}{\Return{$P_\xi$}}
	Find a relative interior point $\mu$ of the optimal facet of~\eqref{facet_problem}\;
	\label{reduce_step}
	\For{$s\in \V$, $t\in\N(s)$, $\xi_{si}=1$, $j\in \L_t$}{ %such that $\mu_{s}(y_s) > 0$
		\lIf{$\mu_{s}(y_s) = 0$, $\mu_{s}(i) > 0$}{
		\label{verification_step1}
		$\xi_{si} := 0$%
		}\;
		\lIf{$\xi_{tj}=0$, $\mu_{st}(y_s,j) = 0$, $\mu_{st}(i,j) > 0$ }{
		\label{verification_step2}
		$\xi_{si} := 0$%
		}\;
		\lIf{$\xi_{tj}=1$, $\mu_{st}(y_s,y_t) = 0$, $\mu_{st}(i,j) > 0$}{
			\label{verification_step3}
			$\xi_{si} := 0$%
		}\;%
		}
	}	
\caption{MaxImprove($f$,$y$)
\label{Alg:generic}}
\end{algorithm}

In step~\ref{facet_step} a linear program is solved to determine whether the current mapping is improving (if $v=0$, \cf~\eqref{L-improving},\eqref{L-improving-rev}). If it is not improving ($v<0$) we need to find a relative interior point in the optimal facet. This point $\mu$ has the property that if $\mu_{s}(i) = 0$ it is guaranteed that there is no optimal solution $\mu'$ such that $\mu'_{s}(i) > 0$ and similarly for the pairwise components. Such $\mu$ can be found by an interior point algorithm.

Steps~\ref{verification_step1},~\ref{verification_step2} and~\ref{verification_step3} decrease $\xi$ and the mapping $P_\xi$ reducing a smaller number of variables is attempted in the next iteration. Clearly, if the algorithm terminates, $P_\xi$ is a $\Lambda$-improving mapping for $f$.


%The relative interior point $\mu$ of the optimal facet fully defines the facet in the following sense. If $\mu_{s}(i)=0$ then there exist no $\mu'$ optimal to ~\eqref{facet_problem} such that $\mu'_{s}(i) > 0$; and similarly for the pairwise components. 

We therefore have the following property
\begin{statement} Let $\mu$ be a strict interior point of $\O$ and $\mu' = P \mu$. Then $P(\O) \subseteq \O$ iff %for $\mu' = P\mu$ there holds $\mu'_{s}(i) > 0 \Rightarrow \mu_s(i) >0$ and $\mu'_{st}(i,j) > 0 \Rightarrow \mu_{st}(i,j) >0$.
\begin{subequations}\label{mu' prop}
\begin{align}
\label{mu'_s prop}
&(\forall s, \forall i) \tab & \mu'_{s}(i)>0 \ &\Rightarrow \mu_{s}(i)>0,\\
\label{mu'_st prop}
&(\forall st, \forall ij) \tab & \mu'_{st}(i,j)>0 \ &\Rightarrow \mu_{st}(i,j)>0.
\end{align}
\end{subequations}
\end{statement}
\begin{proof}
The direction $(P(\O) \subseteq \O)  \Rightarrow ~\eqref{mu' prop}$ is trivial. In the other direction, 
from ~\eqref{mu' prop} and complementary slackness for $\mu$ we conclude that $\mu'$ is optimal to~\eqref{facet_problem}. \todo for any $\mu'' \in \O$ show that $P \mu ''$ satisfies ~\eqref{mu' prop}. %and therefore.
\end{proof}
%
\begin{statement}
%If $\xi$ has not decreased during an iteration then $v=0$.
Conditions in steps \ref{verification_step1}-\ref{verification_step3} determine the maximum $P_\xi$ such that $P_{\xi} (\O) \subseteq \O$.
\end{statement}
\begin{proof}
%If 
On one hand, each of the steps \ref{verification_step1}-\ref{verification_step3} is a sufficient condition to determine that there is no improving mapping with $\xi_{si} = 1$. On the other hand, after verifying all these sufficient conditions we obtain that there holds $P_{\xi} (\O) \subseteq \O$, which is proved as follows.
Let $\mu' = P_\xi \mu$. %We will show that $\<f,\mu\>  = \<f,\mu'\> = 0$. %Assume for contradiction that $\<f,\mu\>  < \<f,\mu'\>$. %Then there exist a node $(s,i)$ such that $\mu'_{s}(i) > 0$ and $\mu_{s}(i) = 0$ 
Let us show implications~\eqref{mu' prop}.
Consider the two possible cases for $\xi_{si}$:
\begin{itemize}
\item $\xi_{si}=0$. In this case $\mu'_{s}(i) = \mu_s(i)$.%Property~\eqref{mu'_s prop} follows from $$
\item $\xi_{si}=1$. In this case $\mu'_{s}(i) = 0$ and $\mu'_{s}(y_s) >0$. It must be $\mu_s(y_s) > 0$, otherwise step~\ref{verification_step1} would have zeroed $\xi_{si}$.
\end{itemize}
It follows that implications~\eqref{mu'_s prop} are satisfied.
Consider the four possible cases for $\xi_{si}, \xi_{tj}$:
\begin{itemize}
\item $\xi_{si}=0$, $\xi_{tj}=0$. In this case $\mu'_{st}(i,j) = \mu_{st}(i,j)$.%Property~\eqref{mu'_s prop} follows from $$
\item $\xi_{si}=1$, $\xi_{tj}=1$. In this case $\mu'_{st}(y_s,y_t) >0$. It must be $\mu_{st}(y_s,y_t) > 0$, otherwise step~\ref{verification_step2} would have zeroed $\xi_t$.
\item $\xi_s=0$, $\xi_t=1$. In this case $\mu'_{st}(i,j) = \mu_{s}(i)\leftbb j{=}y_t\rightbb$. If $\mu'_{st}(i,j)> 0$ then $j=y_t$ and $\mu'_{st}(i,y_t) = \mu_{s}(i)>0$. It must be $\mu_{st}(i,y_t)>0$, otherwise step~\ref{verification_step3} would have zeroed $\xi_t$.
\item $\xi_s=1$, $\xi_t=0$. Symmetric to the above.
\end{itemize}
It follows that implications~\eqref{mu'_st prop} are satisfied. 

\end{proof}

%Let $\mu'$ be optimal to ~\eqref{facet_problem}. Then $\mu'_s(i) \neq 0$ iff $\mu_{s,i} \neq 0$ and $\mu'_{st}(i,j) \neq 0$ iff $\mu_{st,ij} \neq 0$

==> tex/max_improve.tex <==
\section{Maximum Improving Mapping}
\subsection{A Richer Class}

%
%
%
%
%
%
%
%
%

\subsection{The Algorithm}
%
\begin{algorithm}
$\C_s = \L_s$ for all $s$\; % $v:=-1$; $x:=0$; $y':=y$; $\X:=\V$\;
\Repeat{}{%$v = 0$
	%Construct binary energy $\hat g$ from $f$ and $y',\, z$ by~\eqref{Pyz-bar-g-pre}\;
	%\begin{equation}\label{verification_step}
	Construct $P$ from $\C$ according to~\eqref{richer-P T}\;
	Calculate%\\[-0.5em]
	\label{facet_step}
	\begin{equation}\label{facet_problem}
	v = \min_{\mu\in\Lambda} \<f - P\T f,\mu\>% a df sd fdsg dfsg dfsg dfgh df% & &\hspace{5cm}%
	\end{equation}
	\lIf(\tcc*[f]{found improving mapping}){v=0}{\Return{$P$}}
	Find a relative interior point $\mu$ of the optimal facet of~\eqref{facet_problem}\;
	\label{reduce_step}
	\For{$s\in \V$, $t\in\N(s)$, $i\in \C_s$, $j\in \L_t$}{ %such that $\mu_{s}(y_s) > 0$
		\lIf{$\mu_{s}(y_s) = 0$, $\mu_{s}(i) > 0$}{
		\label{verification_step1}
		$\C_s := C_s \backslash\{i\}$%
		}\;
		\lIf{$j\notin C_t$, $\mu_{st}(y_s,j) = 0$, $\mu_{st}(i,j) > 0$ }{
		\label{verification_step2}
		$\C_s := C_s \backslash\{i\}$%
		}\;
		\lIf{$j\in C_t$, $\mu_{st}(y_s,y_t) = 0$, $\mu_{st}(i,j) > 0$}{
			\label{verification_step3}
			$\C_s := C_s \backslash\{i\}$%
		}\;%
		}
	}	
\caption{MaxImprove($f$,$y$)
\label{Alg:generic}}
\end{algorithm}
%
%
%
%
%

==> tex/unification-short.tex <==
\section{Special Cases}\label{S:unification}
The new sufficient condition generalizes several previously proposed sufficient conditions. We will show here improving mappings corresponding to each method. Proofs that the mapping is actually relaxed improving in each case (which is a stronger requirement)~is given in \cite{suppl}.
%\begin{itemize}
%\end{itemize}
\mypar{DEE}
There is a number of local sufficient conditions proposed~\cite{Desmet-92-dee,Goldstein-94-dee}, \etc. %proposed that are generally referred to as {\em dead end elimination} (DEE)~\cite{Desmet-92-dee,Goldstein-94-dee}.
We can show to include Goldstain's simple DEE condition.
%Simple version of methods formulate a 
%variants that are condition to 
%It eliminates label $\alpha$ in pixel $s$ by looking only at terms $f_s$ and $f_{st}$ for $t\in\N(s)$.
The condition allows to eliminate label $\alpha\in\L_s$ if there is label $\beta \in\L_s$ such that replacing $\alpha$ with $\beta$ does not increase the energy for all configurations of neighboring pixels. Clearly, we have the map $p$ which is pixel-wise, it's component $p_t$ is identity for all $t\neq s$ and component $p_s$ has $p_s(\alpha) = \beta$ and $p_s(i) = i$ for $i\neq \alpha$.
%
\mypar{QPBO~\cite{Nemhauser-75,Hammer-84-roof-duality}}
As mentioned above, in the case of 2 lables the LP relaxation has persistency property. The partial assignment of the integral part $(y,\A)$ is globally optimal. Moreover, it has the {\em autarky} property: for any labeling $x$ there holds $\f(x[\A \leftarrow y]) \leq \f(x)$, where $x[\A \leftarrow y]$ is the labeling obtained from $x$ by switching its $\A$ components to $y$~\cite{Boros:TR06-probe}. Clearly, the map $p\colon x \mapsto x[\A \leftarrow y]$ is improving. The relaxed improving property does not hold for autarkies in general, but for the solution of the LP relaxation.
%In this case we have a map $p$ that for no-integral pixels is identity and for integral pixels it replaces any label to the optimal label. It is easy to see that {\em autarky}
%\par
\mypar{MQPBO~\cite{kohli:icml08}}
This method extends partial optimality properties of QPBO to multi-label problems via the reduction of the problem to $0$-$1$ variables. 
%The reduction is for a predefined ordering of labels. 
The method outputs two labelings $x^{\rm min}$ and $x^{\rm max}$ with the guarantee that there exists optimal labeling $x$ that satisfy $x_s \in [x^{\rm min}_s,\, x^{\rm max}_s]$. The improving mapping for this method is given by $p \colon x \mapsto (x \vee x^{\rm min}) \wedge x^{\rm max}$. %Because the reduction is component-wise and we showed component-wise inequalities~\eqref{qpbo-comp} for QPBO, it can be shown that component-wise conditions hold for $p$ and therefore $[p]\in \WI$. (Complete proof in~\cite[\Section{S:mqpbo-s}]{suppl}). %MQPBO method finds a $\Lambda$-improving mapping. The mapping can be written in the form $p(x) = (x \vee x^{\rm min}) \wedge x^{\rm max}$.
%
\mypar{Auxiliary Submodular Problems~\cite{Kovtun03,Kovtun-10}} %In all methods, except of the iterative construction, a {\em test} labeling $y$ is fixed. By constructing an auxiliary submodular problem and finding its minimizer efficiently a set $\A\subset \V$ is found such that $(y_\A,\A)$ is a globally optimal partial assignment. The mapping $p\colon x \mapsto x[\A \leftarrow y]$
%All methods construct an {\em auxiliary} submodular energy $\g$ and its minimizer $x$ .  is selected and a subset $\A\subset\V$ is found such that 
%There are several methods that differ in detail. 
These methods construct an {\em auxiliary} submodular (in a given ordering of labels) energy $\g$. A minimizer $y$ of $\g$ has the property that $\g(x \vee y) \leq \g(x)$, implied by submodularity. It follows that mapping $p\colon x \mapsto x\vee y$ is improving for $g$. 
The construction of the auxiliary function $g$ ensures the inequality $\f(x\vee y) - \f(x) \leq \g(x\vee y)-\g(x)$. It follows immediately that $p$ is improving for $f$. 
%
\mypar{Iterative Pruning~\cite{Swoboda-13}}
This method is applicable to the Potts model and constructs a partial optimal assignment $(\A,y)$.
It turns out that the mapping $p\colon x \mapsto x[\A \leftarrow y]$ is relaxed improving. A recent generalization of this method to arbitrary energies~\cite{Swoboda-14} in the pairwise model satisfies our sufficient condition as well.
%
